Measuring the Prevalence of Anti-Social Behavior in Online Communities

With increasing attention to online anti-social behaviors such as personal attacks and bigotry, it is critical to have an accurate accounting of how widespread anti-social behaviors are. In this paper, we empirically measure the prevalence of anti-social behavior in one of the world's most popular online community platforms. We operationalize this goal as measuring the proportion of unmoderated comments in the 97 most popular communities on Reddit that violate eight widely accepted platform norms. To achieve this goal, we contribute a human-AI pipeline for identifying these violations and a bootstrap sampling method to quantify measurement uncertainty. We find that 6.25% (95% Confidence Interval [5.36%, 7.13%]) of all comments in 2016, and 4.28% (95% CI [2.50%, 6.26%]) in 2020-2021, are violations of these norms. Most anti-social behaviors remain unmoderated: moderators only removed one in twenty violating comments in 2016, and one in ten violating comments in 2020. Personal attacks were the most prevalent category of norm violation; pornography and bigotry were the most likely to be moderated, while politically inflammatory comments and misogyny/vulgarity were the least likely to be moderated. This paper offers a method and set of empirical results for tracking these phenomena as both the social practices (e.g., moderation) and technical practices (e.g., design) evolve.

==> content_minor_revision__Apr2022/figure/bootstrap_workflow.tex <==
\begin{figure}[tb]
  \centering
  \includegraphics[width=1.0\textwidth]{content_minor_revision__Apr2022/images/bootstrap_workflow_6.jpg}
  \caption{\rnr{An overview of the sampling process in broad strokes. We start by randomly sampling unmoderated comments from $T_{2016}$ and $T_{2020}$ to generate our study datasets. We then use these datasets and the annotated comments to calculate key quantities that are needed for our bootstrap resampling. We then combine these quantities to implement our resampling procedure, which we repeat 1,000 times for each time periods of our interest.}}
  \label{fig:bootstrap}
  \Description{Bootstrap resampling workflow}
\end{figure}
